Co-Generation with GANs using AIS based HMC

Inferring the most likely configuration for a subset of variables of a joint distribution given the remaining ones - which we refer to as co-generation - is an important challenge that is computationally demanding for all but the simplest settings. This task has received a considerable amount of attention, particularly for classical ways of modeling distributions like structured prediction. In contrast, almost nothing is known about this task when considering recently proposed techniques for modeling high-dimensional distributions, particularly generative adversarial nets (GANs). Therefore, in this paper, we study the occurring challenges for co-generation with GANs. To address those challenges we develop an annealed importance sampling based Hamiltonian Monte Carlo co-generation algorithm. The presented approach significantly outperforms classical gradient based methods on a synthetic and on the CelebA and LSUN datasets.

==> figs/rel.tex <==
% !TEX root = neurips_2019.tex
\vspace{-0.2cm}
\section{Related Work}
\label{sec:rel}
\vspace{-0.2cm}
In the following, we briefly discuss generative adversarial nets before providing
background on co-generation with adversarial nets.




\noindent\textbf{Generative adversarial nets} (GANs)~\cite{GoodfellowNIPS2014}
have originally been proposed as a non-cooperative two-player game, pitting a
generator against a discriminator. The discriminator is tasked to tell apart
real data from samples produced by the generator, while the generator is asked
to make differentiation for the discriminator as hard as possible. For a dataset
of samples $x\in\cX$ and random perturbations $z$ drawn from a simple
distribution, this intuitive formulation results in the saddle-point objective
$$
\max_\theta\min_w -\mathbb{E}_{{x}}[\ln D_w({x})] - \mathbb{E}_{{z}}[\ln (1-D_w(G_\theta({z})))],
$$
where $G_\theta$ denotes the generator parameterized by $\theta$ and $D_w$
refers to the discriminator parameterized by $w$. The discriminator assesses the probability of  its input argument
being real data. We let $\cX$ denote the output space. % and the latent space.
Subsequently, we refer to this formulation as the `Vanilla GAN,' and note that
its loss is related to the Jensen-Shannon divergence. Many other divergences and
distances have been proposed recently~\cite{arjovsky2017wasserstein,
li2017mmd,gulrajani2017improved,kolouri2017sliced,deshpande2018generative,
cully2017magan,mroueh2017mcgan,berthelot2017began,mroueh2017fisher,
lin2017pacgan,heusel2017gans,salimans2018improving} to improve the stability of the saddle-point
objective optimization during training and to address mode-collapse, some theoretically founded
and others empirically motivated. It is
beyond the scope to review all those variants. 



\noindent\textbf{Co-generation}, is \emph{the task of obtaining a sample for a subset of the output space domain, given as input the remainder of the output
space domain}. This task is useful for applications like image
inpainting~\cite{PathakCVPR2016,YehChenCVPR2017}  or image-to-image
translation~\cite{isola2017,LeeECCV2018,HuangECCV2018,LiuNIPS2017,RoyerARXIV2017,YiICCV2017,cyclegan,ZhuNIPS2017}.
Many formulations for co-generation have been considered in the past. However,
few meet the criteria that \emph{any} given a subset of the output space could be
provided to generate the remainder.

Conditional GANs~\cite{MirzaARXIV2014} have been used to generate output space
objects based on a given input signal~\cite{WangCVPR2018}. The output space
object is typically generated as a whole and, to the best of our knowledge, no
decomposition into multiple subsets is considered.

Co-generation is  related to multi-modal Boltzmann
machines~\cite{SrivastavaNIPS2012,NgiamICML2011}, which learn a shared
representation for video and audio~\cite{NgiamICML2011} or image and
text~\cite{SrivastavaNIPS2012}. Restricted Boltzmann Machine based
encoder-decoder architectures are used to reconstruct either video/audio or
image/text given one of the representations. %These works differ from ours in
%that decoders need to be trained for every subset of the output space domain,
%which is not scalable unless we are interested in a few distinct subsets.
%
Co-generation is also related to deep net based joint embedding space
learning~\cite{KirosARXIV2014}. Specifically, a joint embedding of images and
text into a single vector space is demonstrated using deep net encoders. After performing vector operations in the embedding space, a new sentence can be
constructed using a decoder. 
Co-generation is also related to cross-domain image
generation~\cite{YimCVPR2015,ReedNIPS2015,DosovitskiyCVPR2015,AnooshehARXIV2017}.
Those techniques use  an encoder-decoder style deep net to transform rotation of
faces, to learn the transfer of style properties like rotation and translation to
other objects, or to encode class, view and transformation parameters into
images. 
Image-to-image translation is related in that a transformation between two
domains is learned either via an Image Transformation Net or an Encoder-Decoder
architecture. Early works in this direction tackled supervised image-to-image
translation~\cite{JohnsonECCV2016,isola2017,LedigCVPR2017,ChenICCV2017,LiangARXIV2017,ChoiCVPR2018}
followed by unsupervised
variants~\cite{TaigmanICLR2017,ShrivastavaCVPR2017,YiICCV2017,RoyerARXIV2017,BousmalisCVPR2017,WolfICCV2017,TauICLR2018,HoshenICLR2018}.
Cycle-consistency was discovered as a convenient regularization mechanism
in~\cite{KimICML2017,cyclegan,LiuNIPS2017,AlmahairiARXIV2018} and a distance
preserving regularization was shown by~\citet{BenaimNIPS2017}. Disentangling of
image representations was investigated recently~\cite{HuangECCV2018,LeeECCV2018}
and ambiguity in the task was considered by \citet{ZhuNIPS2017}. Other
losses such as a `triangle formulation' have been investigated
in~\cite{GanNIPS2017,LiXuNIPS2017}.

Attribute transfer~\cite{LaffontTOG2014}, analogy
learning~\cite{HertzmannSIGGRAPH2001,ReedNIPS2015} and many style transfer
approaches~\cite{TenenbaumNIPS1997,BousmalisNIPS2016,VillegasICLR2017,DentonNIPS2017,MathieuNIPS2016,UlyanovICML2016,HuangICCV2017,LiFangNIPS2017,LiECCV2018,TulyakovCVPR2018,DonahueICLR2018,ShenNIPS2017,DumoulinICLR2017,GhiasiBMVC2017,ZhuECCV2016}
just like feature learning via inpainting~\cite{PathakCVPR2016} are also using
an encoder-decoder formulation, which maps entire samples from one domain to
entire samples in another domain.

Co-generation is at least challenging if not impossible for all the
aforementioned works since decoders need to be trained for every subset of the
output space domain. This is not scalable unless we know ahead of time the few
distinct subsets of interest. 
Hence, to generate arbitrary sub-spaces, other techniques need to be considered.
Some applicable exceptions from the encoder-decoder style training are work on
style transfer by \citet{GatysCVPR2016},  work on image inpainting
by \citet{YehChenCVPR2017}, and coupled generative adversarial nets
(CoGANs) by \citet{LiuNIPS2016}. In all three formulations, a loss is optimized  
to match observations to parts of the generated data 
by iteratively computing gradient updates for a latent space sample. 

In particular, \citet{LiuNIPS2016} learn a joint distribution over
multiple domains by coupling multiple generators and possibly discriminators via
weight-sharing. 
\citet{LiuNIPS2016}
briefly discuss co-generation when talking about ``cross-domain image
transformation,'' report to observe coverage issues and state that they leave a
detailed study to ``future work.'' Instead of an optimization based procedure, we
propose to use an annealed importance sampling based  Hamiltonian Monte Carlo
approach. We briefly review both techniques subsequently.

\noindent\textbf{Annealded importance sampling (AIS)}~\cite{NealAIS2001} is an algorithm
typically used to estimate (ratios of) the partition function~\cite{Wuiclr2017,dickhais}. Specifically, it
gradually approaches the partition function for a distribution of interest by
successively refining samples which were initially obtained from a `simple'
distribution, \eg, a multivariate Gaussian. 
Here, we are not interested in the partition function itself, but rather in the
ability of AIS to accurately draw samples from complex distributions, which makes AIS a great tool for co-generation. 

\noindent\textbf{Hamiltonian Monte Carlo (HMC)}~\cite{DuanePLB1987} originally
referred to as ``Hybrid Monte Carlo'' united the Markov Chain Monte
Carlo~\cite{MetropolisCP1953} technique with molecular dynamics
approaches~\cite{Alder1959}. Early on they were used for neural net
models~\cite{NealHMCNeuralNets} and a seminal review by~\citet{NealHMC2010}
provides a detailed account. In short, a Hamiltonian combines the potential
energy, \ie, the log probability that we are interested in sampling from with auxiliary kinetic energy. The latter typically follows a Gaussian distribution.
HMC alternates updates for the kinetic energy with Metropolis updates computed
by following a trajectory of constant value along the Hamiltonian to compute a
new proposal. HMC is useful for co-generation because of its reduced random-walk behavior as we will explain next. 


